Super-resolution Using Constrained Deep Texture Synthesis

Hallucinating high frequency image details in single image super-resolution is a challenging task. Traditional super-resolution methods tend to produce oversmoothed output images due to the ambiguity in mapping between low and high resolution patches. We build on recent success in deep learning based texture synthesis and show that this rich feature space can facilitate successful transfer and synthesis of high frequency image details to improve the visual quality of super-resolution results on a wide variety of natural textures and images.

==> motivation.tex <==

\section{Background and Motivation}
We build on traditional texture synthesis work and  recent advancement of deep learning approaches to experiment with new texture transfer methods that would be useful to example-based image restoration applications, specifically, single image super-resolution and hallucination. Traditional SR methods are conservative in recovering signals due to PSNR considerations and lack the ability to insert image details beyond recoverable limits. The goal of this final chapter is to examine practical ways towards achieving a higher level of photo-realistic appearance while still being perceptually faithful to the input signal constraints. 

\subsection{Traditional Image Priors Tend to Over-smooth}
Natural image content spans a broad range of spatial frequencies, and it is typically easy to constrain the restoration process to reliable recover information in the low frequency bands. These typically include smoothly varying regions without large gradients (textures and edges). In fact, a Gaussian or Laplacian prior would suit well for most image restoration task. This family of image priors have been shown to work in a variety of settings, in \cite{fergus_2006,Levin_2007_reflect,levin_2009,cho_2009,Sun_sr,xu_jia_2010}, to name a few. More advanced prior models have also been developed such as FRAME~\cite{frame_1998}, the Fields of Experts model and its extensions~\cite{foe_2009}. It is known that the filters learned in these higher order models are essentially tuned low high-pass filters~\cite{weiss_freeman_2007}. As a result, no matter how these priors are formulated, they work under the same principle by penalizing high frequency image content, imposing the constraint that ``images should be smooth'' unless required by the image reconstruction constraint. When these priors are universally applied to every pixel location in the image, it is bound to yield over-smoothed output. For image regions where strong signals are present in the (corrupted) observed image (strong edges, salient structures and boundaries), we can expect the image reconstruction constraints to push the solution away from a flat image. But for regions where meaningful signals are almost completely lost due to blur, downsampling and noise, there is nothing for the reconstruction term to latch onto, and the priors would then favor smooth solutions. But smoothness is just another form of blur, which is exactly what we are trying to restore in the first place (such as SR). \\

\subsection{Complex Priors Cannot Insert Textures}
Another problem with current image restoration frameworks is even the most complex and expressive models cannot insert image details and textures. Image priors have evolved from basic two-tap filter responses to statistics on image patches. One of the most complex (hence expressive) model is the GMM patch model from Zoran and Weiss~\cite{Zoran2011}, which works extremely well for deconvolution and denoising. However, as shown in \ref{chap:specificpriors}, the GMM model does not benefit from having better exemplars, nor does it perform well for restoring high frequency image details. In single image SR, one of the most recent leading methods is based on a deep convolutional network~\cite{DeepSR_eccv2014}, which consists of millions of learned parameters. While it outperforms competing methods slightly in term of PSNR and SSIM scores, the improvement in visual quality is minimal. As we will show in Sec~\ref{sec:finalresults}, the recent state-of-the-art SRCNN method produces nearly visually identical results compared to ScSR~\cite{yang_sr_2008}, a widely cited sparse coding based approach from 2008. With considerable amount of active effort and progress in the recent years, hallucinating and synthesizing visually plausible image details in restored results remains a challenging problem, even for the most successful SR methods. In order to allow better detail synthesis and insertion, maybe it is helpful to consider a different route, and cast the restoration problem as a constrained detail synthesis problem.

\subsection{Texture Related Techniques from Graphics}
Outside of the realm of image restoration, works in the graphics community have examined the task of texture synthesis and manipulation with great success. By taking on a non-parametric approach, simple copy-paste inspired techniques are able to produce visually pleasant image details in various application settings~\cite{efros_leung_99,patchmatch,patchmatch2,imagemelding}. But why do results from these systems look so much more photo-realistic than typical output images in the image restoration literature? We believe there are three fundamental reasons. First, the constraints are different. Almost all image restoration methods require a well-defined image formation model (\eg linear operator with additive Gaussian noise), which is typically regularized by a carefully chosen prior term. But for texture synthesis, there is little constraint on the global appearance of the output image. In image editing and retargetting, there can often be highly specific constraints involving salient structures, straight lines, and mask, but these are typically local constraints, and user-defined. Second, the starting point is different. Image restoration problems usually start from globally corrupted signals, namely, every local patch in the input image requires restoration. However, texture transfer/synthesis work always start with clean and sharp images free of artifacts, hence the algorithm has a better source image to manipulate, and high quality outputs can be expected. Finally, the end goals are different. The quality of restored images have been traditionally measured against a ground truth image by PSNR and SSIM scores, which penalizes any signal that deviates from the ground truth, even if it represents plausible and appropriate image details. However, there are many situations where there exists no single best output image, and any plausible restoration or hallucination of image details should be favored, instead of being penalized due to having high frequency content. \\
We believe that in order to further advance the field of image restoration research, it is beneficial to consider a different direction, where texture transfer is used as the driving force in the restoration process.





